Non-linear Multitask Learning with Deep Gaussian Processes

We present a multi-task learning formulation for Deep Gaussian processes (DGPs), through non-linear mixtures of latent processes. The latent space is composed of private processes that capture within-task information and shared processes that capture across-task dependencies. We propose two different methods for segmenting the latent space: through hard coding shared and task-specific processes or through soft sharing with Automatic Relevance Determination kernels. We show that our formulation is able to improve the learning performance and transfer information between the tasks, outperforming other probabilistic multi-task learning models across real-world and benchmarking settings.

==> sections/relationship_to_other_models.tex <==
\section{LINK TO OTHER MODELS}
In this section, we briefly explore the connection of the proposed model to other models in the multi-task learning literature.
\subsection{Linear Process Mixing}
To make the relationship of the proposed model to other GP-based models more explicit, we consider the following construction of a multi-output function $f(x)$ of $T$ outputs, where we refer to the $t$th output as
\begin{equation}
    f^t(\mathbf{x}) = \sum_{i=1}^I w^t_i g_j(\mathbf{x}) + \sum_{j=i}^J h^t_j(\mathbf{x}),
    \label{eqn:linear-basis}
\end{equation}
where $\{w_i^t\}_{i=1}^I$ is a set of weights associated with output $t$, and the $g_j(\cdot)$'s and $h^t_j(\cdot)$ are basis functions that are shared and output specific, respectively. In the probabilistic literature, the set of basis functions are modelled as independent GPs with their choice of covariance function determining the particular model, e.g. setting independent GP priors on the basis functions with different covariance functions recovers the Semi-parametric Latent Factor Model of \citet{whye_teh_semiparametric_2005}. Since, the output processes are a sum of GPs, it follows that they themselves are also GPs with tractable cross-cavariance that depends on the weights on the shared basis functions.

We can generalise the construction in \cref{eqn:linear-basis} to the following:
\begin{equation}
    f^t(\mathbf{x}) = \varphi^t(g_1(\mathbf{x}), \dots, g_I(\mathbf{x}), h_1^t(\mathbf{x}), \dots, h_J^t(\mathbf{x})),
    \label{eqn:composition}
\end{equation}
where $\varphi^t(\cdot)$ is an arbitrary function. Depending on the choice of $\varphi^t(\cdot)$, this construction combines the basis functions non-linearly; for instance, allowing interactions between the shared and output specific processes. Treating this construction probabilistically, we can place GP priors on the basis function as well as the warping function $\varphi^t(\cdot)$, which recovers the proposed model. It is important to note that due to the non-linearity of $\varphi^t(\cdot)$, the resulting output processes are no longer Gaussian and, for all but the simplest cases, their cross-covariance cannot be characterised in terms of the shared basis functions only. As a side note, choosing a GP with linear covariance function as a prior on $\varphi^t(\cdot)$ recovers the linear model described in \cref{eqn:linear-basis}.

\subsection{Process Convolution}
One can formulate a GP as the convolution of a base process with a smoothing kernel, i.e.
\begin{equation}
    f(\mathbf{z}) = \int_\chi G(\mathbf{x} - \mathbf{z})u(\mathbf{z})d\mathbf{z},
    \label{eqn:convolution}
\end{equation}
where the smoothing kernel $G(\cdot)$ is square integrable (i.e. $\int G^2(x-u)du < \infty$) and the base process $u(\cdot)$ is a white noise process, or more generally any random process (although if non-Gaussian then the resulting convolution process is not a GP) \citep{calder2007some}. In the multi-output process convolution literature, different outputs are assumed to share the same base process $u$, with different smoothing kernels for each output. Hence, the cross-covariance between the output process can be derived tractably since the convolution is a linear operation.

Using \cref{eqn:convolution} and conditioned on the latent processes, we can write the top layer of the presented model as
\begin{equation}
    f^t(\mathbf{x}) = \int_\chi G^t(\mathbf{g} - \mathbf{z}_g, \mathbf{h}^t - \mathbf{z}_h)u^t(\mathbf{z})d\mathbf{z},
    \label{eqn:mtl-convolution1}
\end{equation}
assuming a separable smoothing kernel $G^t(\mathbf{g} - \mathbf{z}_g, \mathbf{h}^t - \mathbf{z}_h) = G^t(\mathbf{g} - \mathbf{z}_g) G^t( \mathbf{h}^t - \mathbf{z}_h)$ (which will be the case for processes with ARD kernels), we can rewrite \cref{eqn:mtl-convolution1} as
\begin{align}
    f^t(\mathbf{x}) =& \int_\chi G^t(\mathbf{g} - \mathbf{z}_g)G^t( \mathbf{h}^t - \mathbf{z}_h)u^t(\mathbf{z})d\mathbf{z} \nonumber \\
    =& \int_\chi G^t(\mathbf{g} - \mathbf{z}_g)\upsilon^t(\mathbf{z}_g)d\mathbf{z}_g,
    \label{eqn:mtl-convolution2}
\end{align}
where $\upsilon^t$ is also random process. Since by construction, $g$ itself is a random (Gaussian) process, we can see that the output correlation is induced in the smoothing kernel rather than the base process. Conditioning the smoothing kernel on a random process is an explored idea to induce non-stationary behaviour in the output process \citep{higdon1998process, higdon1999non}; however, to the best of our knowledge this work is the first instance to consider this for information sharing behaviour.

\subsection{Regularisation Methods}
The ELBO defined in \cref{eqn:mtl-elbo} has a similar formulation to the general multi-task objective function in regularisation-based multi-task learning literature \citep{evgeniou2004regularized}. A general formulation of which is given by
\begin{equation}
    \label{eqn:mtl-objective}
    \frac{1}{T} \sum_{t=1}^T L^t(\theta, \phi; \mathbf{Y}^t) + \Omega(\theta) + \sum_{t=1}^T\Psi(\phi^t),
\end{equation}
where $\theta$ are shared parameters, $\phi = \{\phi^t\}_{t=1}^T$ are task specific parameters and $\{L\}_{t=1}^T$, $\Omega$ and $\{\Psi\}_{t=1}^T$ are the task specific losses, shared regulariser and task specific regularisers respectively. In this setting, the choice and strength of regularisation controls the information transfer between the tasks.

A direct analogy can be drawn from \cref{eqn:mtl-elbo} to \cref{eqn:mtl-objective}, where the expected log-likelihood terms correspond to the loss functions and the KL terms correspond to the regularisers, respectively. This forms a new link between the probabilistic and the regularisation points-of-view of multi-task learning and motivates the prospect of choosing alternative prior processes to induce desirable behaviour in the model such as sparsity in the latent space \cite{argyriou2007multi}. Furthermore, one can also frame \cref{eqn:mtl-elbo} as a Generalised Variational Inference objective  \citep{knoblauch2019generalized}, where the KL terms are viewed as prior regularisers. Changing the form of these regularisers can induce different information sharing behaviours in the approximate predictive posteriors of the tasks. Unfortunately, exploring this point further is beyond the scope of this work.

==> sections/robustification.tex <==
\section{ROBUST MULTITASK DGPs}
The ELBO defined in \cref{eqn:mtl-elbo} has a similar formulation to the general multi-task objective function in regularisation-based multi-task learning literature \citep{evgeniou2004regularized}. A general formulation of which is given by
\begin{equation}
    \label{eqn:mtl-objective}
    \frac{1}{T} \sum_{t=1}^T L^t(\theta, \phi; \mathbf{Y}^t) + \Omega(\theta) + \sum_{t=1}^T\Psi(\phi^t),
\end{equation}
where $\theta$ are shared parameters, $\phi = \{\phi^t\}_{t=1}^T$ are task specific parameters and $\{L\}_{t=1}^T$, $\Omega$ and $\{\Psi\}_{t=1}^T$ are the task specific losses, shared regulariser and task specific regularisers respectively. In this setting, the choice and strength of regularisation controls the information transfer between the tasks.

A direct analogy can be drawn from \cref{eqn:mtl-elbo} to \cref{eqn:mtl-objective}, where the expected log-likelihood terms correspond to the loss functions and the KL terms correspond to the regularisers, respectively. This can be justified by framing the negative of the ELBO in \cref{eqn:mtl-elbo} as a Generalized Variational Inference (GVI) objective \citep{knoblauch2019generalized}.\theo{I think we would need to pull more math from GVI/Robust DGP angle in here to better describe it and also beef up the technical appearance of the paper. Also need to pull some short technical link to the Composite likelihood link and work by Holmes.}

The correspondence between the two objectives motivates the modification of the uncertainty regularisers in the GVI objective to control the information transfer in the proposed model. While, any admissible divergence can be used to modify the objective \citep{knoblauch2019generalized}, we propose the following simple modification to \cref{eqn:mtl-elbo}:
\begin{align}
\mathcal{L} =& \sum_{t=1}^T \sum_{n=1}^{N^t} \mathbb{E}_{q(\mathbf{f}_n^t)}[\log p(\mathbf{y}_n^t | \mathbf{f}_n^t)] 
\color{blue} - \sum_{t=1}^T \alpha^t\text{KL}\left[q(\mathbf{\tilde{F}}^t) \middle\| p(\mathbf{\tilde{F}}^t)\right] \nonumber \\
&\color{green} - \sum_{t=1}^T \sum_{j=1}^{J^t} \gamma_j^t\text{KL}\left[q(\mathbf{\tilde{H}}^t_j) \middle\| p(\mathbf{\tilde{H}}_j^t)\right]
\color{red} -\sum_{i=1}^I \beta_i\text{KL}\left[q(\mathbf{\tilde{G}}_i) \middle\| p(\mathbf{\tilde{G}}_i)\right],  \label{eqn:mtl-gvi-elbo}
\end{align}
where $\{\alpha^t\}_{t=1}^T$, $\{\beta_i\}$ and $\{\gamma_j^t\}$ are scalar parameters that control the strength of the regularisation against the prior for the corresponding model components.

Introducing the ability to control the prior regularisation in the inference objective allows us to bias the approximate posterior solution towards more desired properties in a similar fashion to the disentanglement problem considered in \citet{higgins2017beta}. In the multi-task setting, we desire solutions that prefer maximal information sharing between tasks. To this end, upweighting the task specific regulariser acts as an information bottleneck on the task specific components of the model. This in turn encourages the shared component to absorb information maximally. 

Note that the objective in \cref{eqn:mtl-gvi-elbo} can no longer be interpreted as a lower bound on the model evidence. However, {\color{red}justification for use in model selection ...}

To further justify our choice of objective, we make the following conjectures:
\begin{enumerate}
    \item C1: The mean-field approach to approximating the DGP posterior of \citet{titsias_variational_2009} fails to take into account the posterior covariance between latent processes. This is especially the case in our formulation where one would expect posterior coupling between the shared and task specific processes of the middle layer.
    \item C2: In black-box multi-task modelling, we are operating in a regime where our model is almost always misspecified.
\end{enumerate}
For all but the simplest cases, C1 implies that the true posterior is unlikely to be contained within the chosen approximation family. Even if it was, C2 implies that the true posterior might not be desirable in a decision theoretic point-of-view if the end goal of the modelling process is purely predictive.\theo{Need to be stronger in this section in terms of the lower bound interpretation etc - Also paper needs pseudo-algorithm, especially if the weights stay}
